On polynomial explicit partial estimator design for nonlinear systems with parametric uncertainties

This paper investigates the idea of designing data-driven partial estimators for nonlinear systems showing parametric uncertainties using sparse multivariate polynomial relationships. A general framework is first presented and then validated on two illustrative examples with comparison to different possible Machine/Deep-Learning based alternatives. The results suggests the superiority of the proposed sparse identification scheme, at least when the learning data is small.

==> dfe_train_noise_0.tex <==
\begin{tabular}{lrrrr}
\toprule
$q$ & n=1 & n=2 & n=3 & n=4 \\
\midrule
50\% & 0.36 & 1.12 & \textbf{0.01} & 0.25 \\
80\% & 0.92 & 1.77 & \textbf{0.01} & 0.56 \\
90\% & 1.75 & 2.81 & \textbf{0.03} & 0.88 \\
95\% & 3.57 & 4.82 & \textbf{0.05} & 1.54 \\
98\% & 7.31 & 8.03 & \textbf{0.08} & 2.63 \\
99\% & 9.28 & 10.96 & \textbf{0.10} & 3.30 \\
100\% & 18.69 & 26.92 & \textbf{0.17} & 7.76 \\
\bottomrule
\end{tabular}


==> dfe_train_noise_03.tex <==
\begin{tabular}{lrrrr}
\toprule
$q$ & n=1 & n=2 & n=3 & n=4 \\
\midrule
50\% & 0.45 & 1.32 & \textbf{0.01} & 0.49 \\
80\% & 1.11 & 2.01 & \textbf{0.04} & 1.04 \\
90\% & 1.89 & 3.26 & \textbf{0.06} & 1.79 \\
95\% & 3.58 & 5.52 & \textbf{0.08} & 2.75 \\
98\% & 7.34 & 8.99 & \textbf{0.11} & 4.78 \\
99\% & 9.21 & 11.78 & \textbf{0.12} & 6.16 \\
100\% & 18.41 & 28.33 & \textbf{0.82} & 37.01 \\
\bottomrule
\end{tabular}


==> dftest.tex <==
\begin{tabular}{lrrrrrrr}
\toprule
$q$ & 50\% & 80\% & 90\% & 95\% & 98\% & 99\% & 100\% \\
\midrule
Error & \textbf{0.01} & \textbf{0.03} & \textbf{0.04} & \textbf{0.06} & \textbf{0.12} & \textbf{0.22} & \textbf{1.46} \\
\bottomrule
\end{tabular}


==> dftest_d1.tex <==
\begin{tabular}{lrrrrrrr}
\toprule
q & 50\% & 80\% & 90\% & 95\% & 98\% & 99\% & 100\% \\
\midrule
Error & 0.03 & 0.07 & 0.09 & 0.13 & 0.24 & 0.36 & 1.82 \\
\bottomrule
\end{tabular}
